Multilingual Pretraining Using a Large Corpus Machine-Translated from a Single Source Language

English, as a very high-resource language, enables the pretraining of high-quality large language models (LLMs). The same cannot be said for most other languages, as leading LLMs still underperform for non-English languages, likely due to a gap in the quality and diversity of the available multilingual pretraining corpora. In this work, we find that machine-translated text from a single high-quality source language can contribute significantly to the pretraining of multilingual LLMs. We translate FineWeb-Edu, a high-quality English web dataset, into French, German, and Spanish, resulting in a final 300B-token dataset, which we call TransWeb-Edu, and pretrain a 1.3B-parameter model, CuatroLLM, from scratch on this dataset. Across five non-English reasoning tasks, we show that CuatroLLM matches or outperforms state-of-the-art multilingual models trained using closed data, such as Llama3.2 and Gemma2, despite using an order of magnitude less data, such as about 6% of the tokens used for Llama3.2's training. We further demonstrate that with additional domain-specific pretraining, amounting to less than 1% of TransWeb-Edu, CuatroLLM surpasses the state of the art in multilingual reasoning. To promote reproducibility, we release our corpus, models, and training pipeline under open licenses at hf.co/britllm/CuatroLLM.

==> tables/variance-figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{tables/arc-bar.pdf}
    % \includegraphics[width=0.8\columnwidth]{img/fig1}
    % \includegraphics[width=0.8\columnwidth]{tables/arc.pdf}
    % \includegraphics[width=0.4\columnwidth]{img/fig1_subj_2shot}


    \caption{ARC variance
    }
\end{figure}
